Uncertain Spatial Data Management:An Overview

Both the current trends in technology such as smartphones, general mobile devices, stationary sensors, and satellites as well as a new user mentality of using this technology to voluntarily share enriched location information produces a flood of geo-spatial and geo-spatiotemporal data. This data flood provides tremendous potential for discovering new and useful knowledge. But in addition to the fact that measurements are imprecise, spatial data is often interpolated between discrete observations. To reduce communication and bandwidth utilization, data is often subjected to a reduction, thereby eliminating some of the known/recorded values. These issues introduce the notion of uncertainty in spatial data management, an aspect raising the imminent need for scalable and flexible solutions. The main scope of this chapter is to survey existing techniques for managing, querying, and mining uncertain spatial data. First, this chapter surveys common data representations for uncertain data, explains the commonly used possible worlds semantics to interpret an uncertain database, and surveys existing system to process uncertain data. Then, this chapter defines the notion of probabilistic result semantics to distinguish the task of computing individual object probabilities versus computing entire result probabilities. This is important, as, for many queries, the problem of computing object-level probabilities can be solved efficiently, whereas result-level probabilities are hard to compute. Finally, this chapter introduces a novel paradigm to efficiently answer any kind of query on uncertain data: the Paradigm of Equivalent Worlds, which groups the exponential set of possible database worlds into a polynomial number of sets of equivalent worlds that can be processed efficiently. Examples and use-cases of querying uncertain spatial data are provided using the example of uncertain range queries.

==> sec_continuous.tex <==
\subsection{The PCNN Query}
%In certain trajectory databases, \textit{continuous} nearest neighbour queries
%are often the matter of choice. Given an input trajectory $T_q$ and a query
%interval $[s,e]$, such continuous queries return a set of tuples $(o_1, i_1),
%\ldots, (o_n, i_n)$ with $\mathop{\cup}\limits_{j=1\ldots n} i_i= [s,e]$, such
%that for each of these tuples there is $\forall_j:\forall_t \in i_j: o_n = NN(q)$.
%\cite{papadias etc}.

% The PCNNQ as defined in Section \ref{subsec:querydef} extends the
% traditional CNN query \cite{PraWolChaDao97, TaoPapShe02} that
% retrieves the nearest neighbor of every point on a given query
% trajectory to uncertain trajectory data. A first approach for
% extending the CNN problem to uncertain spatio-temporal databases
% has been proposed in \cite{TraTamCruSchHarZam11} where efficient solutions for this
% problem have been investigated for the case where temporal
% dependencies are not taken into account. In this section we will
% demonstrate that the general PCNNQ problem is hard if temporal
% dependencies are taken into account.

%Let us first consider an instance of a direct mapping of the certain CNN problem
%to our probabilistic setting under temporal dependencies, denoted as $PCNN$ in
%the following.
%\begin{definition}{PCNN query}
%  Given a spatio-temporal exact Object \query, a spatial location \loc, a time
%  interval $\tint= [\tint_0, \tint_1]$ and a set of probabilistic objects \db, a
%  PCNN query returns, for each object $x \in \DB$ all tuples $(T_x, P_x)$ with
%  $T_x \subseteq \tint$, $P_x = P\forall NN(\query, \db, T_x), P_x > 0$.
%\end{definition}

The traditional CNN query \cite{PraWolChaDao97, TaoPapShe02}, retrieves the
nearest neighbor of every point on a given query trajectory in a time interval
$T$. This basic definition usually returns $m << |T|$ time intervals together
having the same nearest neighbor. The main issue when considering uncertain
trajectories and extending the query definition is the possibly large number of
results due to highly overlapping and alternating result intervals. In
particular, considering Definition \ref{def:ustnnpcnnq}, a PCNN result may have an
exponential number of elements when $\tau$ becomes small. This is because in the
worst case each $T_i\subseteq T$ can be associated with an object $o$ for which the probability
$P\forall NN(o,q,\DB,T_i)\geq\tau$, i.e., $2^T$ different $T_i$'s occur in the
result set.

To alleviate (but not solve) this issue, in the following
we propose a technique based on Apriori pattern mining to return the subsets of $T$ that have
a probability greater than $\tau$. This algorithm requires to compute a
$P\forall NN$ probability in each validation step; we assume that this is
achieved by employing the sampling approach proposed in
Section~\ref{chap:sampling}.
Since each subset of $T$ may have a probability greater than $\tau$ (especially when $\tau$ is chosen too small), a worst-case
of $O(2^n)$ validations may have to be performed.

\textbf{Algorithm. }% \label{subsec:PCNN_algorithm}
Algorithm \ref{alg:PCNN} shows how to compute, for a query trajectory $q$, a
time interval $T$, a probability threshold $\tau$, and an uncertain trajectory
$o\in\DB$ all $T_i \subseteq T$ for which $o$ is the nearest neighbor to $q$ at
all timestamps in $T_i$ with probability of at least $\tau$, and the
corresponding probabilities.

%\begin{algorithm}
%  \caption{$PCNNQ(q,\DB,T,\tau)$}
%  \begin{algorithmic}[1]
%    \label{alg:PCNNQ}
%        \STATE result = $\emptyset$
%        \FOR{$o\in\DB$}
%            \STATE result = result $\cup \{(o,PC_\tau NN(q,o,\DB,T,\tau))\}$
%        \ENDFOR
%        \RETURN result
%  \end{algorithmic}
%%  \vspace{-0.1cm}
%\end{algorithm}


  \begin{algorithm}
  \small
  \caption{$PC_\tau NN$($q$, $o$, $\DB$, T, $\tau$)}
  \begin{algorithmic}[1]
    \label{alg:PCtauNN}
        \STATE $L_1 = \{(\{\tint\},P)| \tint\in T \wedge P=P\forall
        NN(o,q,\DB\setminus\{o\}, \{\tint\}) \geq \tau\}$ \label{alg:PCNN_L1}
        \FOR{$k=2; L_{k-1}\not = \emptyset; k++$} \label{alg:PCNN_L2}
          %\STATE $X^k = \{T_k\subseteq T_i| |T_k|=k\wedge\exists(T_{k-1},p)\in
          % L_{k-1}:T_{k-1}\subset T_k\}$ \label{alg:PCNN_L3}
          \STATE $X^k = \{T_k\subseteq T| |T_k|=k\wedge \forall T'_{k-1} \subset
          T_k \exists (T'_{k-1}, P) \in L_{k-1}\}$ \label{alg:PCNN_L3}
          \STATE $L_k = \{(T_k,P) | T_k\in X^k \wedge P=P\forall
          NN(o,q,\DB\setminus\{o\},T_k) \ge \tau\}$\label{alg:PCNN_L4}
        \ENDFOR
        \RETURN $\bigcup_k L_k$ \label{alg:PCNN_L7}
  \end{algorithmic}
  \label{alg:PCNN}
 % \vspace{-0.1cm}
\end{algorithm}


We take advantage of the anti-monotonicity property that for a $T_i$ to
qualify as a result of the PCNNQ query, all proper subsets of $T_i$ must also
satisfy this query. In other words if $o$ is the P$\forall$NN of $q$
in $T_i$ with probability at least $\tau$, then for all $T_j\subset T_i$
$o$ must be the P$\forall$NN of $q$ in $T_j$ with
probability at least $\tau$.
Exploiting this property, we adapt the Apriori pattern-mining approach from
\cite{AgrSri94} to solve the problem as follows.
We start by computing the probabilities of all single points of time
to be query results (line~\ref{alg:PCNN_L1}).
Then, we iteratively consider the set $X^k$ of all timestamp sets with $k$
points of time by extending timestamp sets $T_{k-1}$ with an
additional point of time $t\in T\setminus T_{k-1}$, such that all $T'_{k-1}
\subset T_k$ have qualified at the previous iteration, i.e., we have $P\forall
NN(o,q,\DB\setminus\{o\},T'_{k-1}))\geq\tau$ (line~\ref{alg:PCNN_L3}).

%DO NOT REMOVE THIS PRAGRAPH (newline) AS IT WAS REQUESTED BY REVIEWER 2
The P$\forall$NN probability is monotonically decreasing with the number of
points in time considered, i.e.,
P$\forall$NN($o,q,\DB\setminus\{o\},T_k$) $\ge$
P$\forall$NN($\query,\DB,T_{k+1}$) where $T_{k}\subset T_{k+1}$.
Therefore we do not have to further consider the set of points of time $T_k$
that do not qualify for the next iterations during the iterative construction of
sets of time points. Based on the sets of timesteps $T_k$ constructed in
each iteration we compute $P\forall
NN(o,q,\DB\setminus\{o\},T_k)$ to build the set of results of length $k$ (line~\ref{alg:PCNN_L4}) that are finally collected and reported as result
in line~\ref{alg:PCNN_L7}. The basic algorithm can be sped up by employing the
property that given P$\forall$NN($o,q,\DB\setminus\{o\},T_1) =1$ the probability of P$\forall$NN($o,q,\DB\setminus\{o\},T_1 \cup T_2) =$
P$\forall$NN($o,q,\DB\setminus\{o\}, T_2)$.

Based on Algorithm \ref{alg:PCtauNN} it is possible to define a straightforward
algorithm for processing PCNNQ queries (by considering each object $o'$ from the
database). 

%During this iterative construction, let the set of tuples $L_{k-1}$, containing
%tuples $(\tint_{k-1}, p)$ with $|\tint_{k-1}| = k-1 \wedge p > \tau$ be given.
%From these intervals we construct new intervals of length $k$ by
%generating $T_k = \{\tint_k| \forall \tint_i: |\tint_i| = k-1: (\tint_i, p) \in
%L_{k-1}\}$ in line \ref{alg:PCNN_L3}. The set $T_k$ therefore contains sets of
%points in time where each subset is a frequent itemset of length $k-1$. These sets are considered as
%candidates of frequent itemsets of length $k$ that are determined in line
%\ref{alg:PCNN_L4} equivalently to the atomic frequent itemsets in line
%\label{alg:PCNN_L1}. The algorithm terminates if no frequent itemsets of length
%$k$ can be found, i.e. $L_{k} = \emptyset$.
%After terminating, the algorithm returns all tuples $L_k$ with $k \ge 1$.

%WARNUNG: PRUNERS KÖNNEN KANDIDATEN WERDEN, WENN DAS
%ANFRAGEINTERVALL NICHT ZUSAMMENHÄNGEN IST (WIR MACHEN
%INDEX-PRUNING MIT ZUSAMMENHÄNGENDEN INTERVALLEN!)
%In a nutshell, the algorithm from \cite{} splits the query interval into
% several subintervals following the semantics of the certain setting, sucht that for each
%subinterval the following expression holds:
%\[\forall_j:\forall_t \in i_j:\forall_k p(o_j = NN(q)) > p(o_k = NN(q))\]
%Clearly, in this expression, temporal dependencies are not taken into account
%because different points in time are considered independently. Therefore we
% have to adapt the semantics of such a query to fit temporal dependencies.

%To generate results in accordance of the possible worlds semantics taking the
%temporal dependencies into account, we have to follow the following definition:

%\begin{definition}{P-CNN-TD Query}
%Given a database of uncertain objects $\DB$, a query object $q$, and a time
%interval $[s,e]$, a continuous probabilistic nearest neighbour
%query considering temporal dependencies ($P-CNN-TD$ query) returns for each
%object $o_i \in \DB$ a function $f(o, \DB, t)$, such that
%\[f(o, \DB, t) = p(NN(q^t) = o^t)\]
%\end{definition}
%Wir geben ~ unsichere intervalle zurück, pdf gibt wahrscheinlichkeit eines
% schnittes mit dem intervall an.

%While answering such a query quite easily, it is quite difficult to return the
%corresponding result functions $f(o)$ in a useful order. One possibility here
%would be to rank the objects according to $\int_x=s^e f(o) \text{d}x$, which
%would return the object with the highest expected probability of beeing nearest
%neighbour of $q$, however ignoring possible world semantics






==> sec_generatingFunctions.tex <==


\label{GeneratingFunctions} Given a set of $N$ independent but not
necessarily identically distributed Bernoulli $\{0,1\}$ random
variables $X_i,1\leq i \leq N$. Let $P_{LB}(X_i)$ ($P_{UB}(X_i)$)
be a lower (upper) bound approximation of the probability
$P(X_i=1)$. Consider the random variable
$$
\sum_{i=1}^{N}X_i.
$$
We make the following observation: The lower and upper bound
probabilities $P_{LB}(X_i)$ and $P_{UB}(X_i)$ correspond to the
probabilities of the three following events:
\begin{itemize}
\item $X_i=1$ definitely holds with a probability of at least $P_{LB}(A_i\prec_R B)$.

\item $X_i=0$ definitely holds with a probability of at least
$1-P_{UB}(X_i)$.

\item It is unknown whether $X_i=0$ or $X_i=1$ with the remaining
probability of $P_{UB}(A_i\prec_R B)-P_{LB}(A_i\prec_R B)$
$=P_{UB}(A_i\prec_R B)-P_{LB}(A_i\prec_R B)$.
\end{itemize}

Based on this observation, we consider the following uncertain
generating function (UGF):

$$
{\cal{F}}^N=\prod_{i \in 1,...,N}[(P_{LB}(X_i)\cdot x +
(1-P_{UB}(X_i))\cdot y+
$$\vspace{-0.3cm}
$$
(P_{UB}(X_i)-P_{LB}(X_i)))] = \sum_{i,j\geq 0}c_{i,j}x^i y^j.
$$

The coefficient $c_{i,j}$ has the following meaning: With a
probability of $c_{i,j}$, $B$ is definitely dominated at least $i$
times, and possibly dominated another $0$ to $j$ times. Therefore,
the minimum probability that $\sum_{i=1}^{N}X_i=k$ is $c_{k,0}$,
since that is the probability that exactly $k$ random variables
$X_i$ are $1$. The maximum probability that $\sum_{i=1}^{N}X_i=k$
is $\sum_{i\leq k,i+j\geq k}c_{i,j}$, i.e. the total probability
of all possible combinations in which $\sum_{i=1}^{N}X_i=k$, may
hold. Therefore, we obtain an approximated PDF of
$\sum_{i=1}^{N}X_i$. In the approximated PDF of
$\sum_{i=1}^{N}X_i$, each probability $\sum_{i=1}^{N}X_i=k$ is
given by a conservative and a progressive approximation.

\begin{example}
\label{ex:UGF} Let $P_{LB}(X_1)=20\%$, $P_{UB}(X_1)=50\%$,
$P_{LB}(X_2)=60\%$ and $P_{UB}(X_2)=80\%$. The generating function
for the random variable $\sum_{i=1}^{2}X_i$ is the following:
$$
{\cal{F}}^2=(0.2x+0.3y+0.5)(0.6x+0.2y+0.2)$$\vspace{-0.6cm}
$$=0.12x^2+0.34x+0.1+0.22xy+0.16y+0.06y^2
$$
That implies that, with a probability of at least $12\%$,
$\sum_{i=1}^{2}X_i=2$. In addition, with a probability of $22\%$
plus $6\%$, it may hold that $\sum_{i=1}^{2}X_i=2$, so that we
obtain a probability bound of $12\%-40\%$ for the random event
$\sum_{i=1}^{2}X_i=2$. Analogously, $\sum_{i=1}^{2}X_i=1$ with a
probability of $34\%-78\%$ and $\sum_{i=1}^{2}X_i=0$ with a
probability of $10\%-32\%$. The approximated PDF of
$\sum_{i=1}^{2}X_i$ is depicted in Figure
\ref{fig:approximatePDF}.
\end{example}

\begin{figure}[ht]
    \centering
    \includegraphics[width = 0.75\columnwidth]{figures/approxPDF.pdf}
    \caption{Approximated PDF of $\sum_{i=1}^{2}X_i$.}
  \label{fig:approximatePDF}
\end{figure}


==> sec_sampling.tex <==
\vspace{-0.2cm}
\section{Probabilistic Spatial Query Processing using Monte-Carlo Sampling}\label{sec:sampling}
A different paradigm to answer queries on uncertain spatial data is Monte-Carlo sampling. In a nutshell, the idea is to sample possible worlds from an uncertain database as described in Section~\ref{sec:pws} and apply a query predicate on each sampled world. If these samples are obtained without bias, meaning that the probability $P_S(\omega)$ of sampling a possible world $\omega\in\Omega$ equals the probability $P(\Omega)$ of the possible worlds, then the results on the sampled worlds can be used as an unbiased estimator of possible results. 
This sampling paradigm for uncertain query processing has been first proposed in~\cite{jampani2008mcdb}. The main drawback of this approach is that the number of possible results may be exponentially large. Thus, it is quite possible that a query may result different results in all or most possible worlds, yielding tiny and equal estimated probabilities for each result. To aggregate possible worlds into groups of mutually similar worlds (having similar results for the query predicate), an approach has been proposed recently~\cite{Schmid2019Representative}


We note that all uncertainty models assuming independence between objects can be sampled without bias, simply by sampling each database object individually. 



This paper targets the problem of efficiently deriving query results and their confidence values from an uncertain dataset. Therefore, we propose a sampling-based solution to query uncertain data which is generally applicable to all data domains and with any uncertain data model, allowing the application of any existing query algorithm, originally designed for certain
  data. Unlike any previous work, our
  approach also considers
  any dependencies between objects.
   Rather than returning exact result probabilities which conforms to all possible worlds, we propose to sample a subset of possible worlds. On each sampled world, we apply a traditional query. Then, the main contribution of this work is to unify the set of sampled query results into a smaller set of \emph{representative query results}. A representative query result is a query result, for which we can guarantee, at a specified level of significance, that the true (but unknown) query result must be similar to this result.




A general approach that is applicable to any uncertainty model is MCDB \cite{JamXufWumPerEtAl11}. Like our approach, MCDB uses Monte-Carlo sampling of possible worlds in order to approximate the result of a given query predicate on. The difference to our approach is how the result sets are handled. For each object, MCDB estimates the probability of each object to be part of the result set. As discussed in Section \ref{sec:introduction}, this is where our approach gains merit: By considering the result sets as a whole, and by finding representative result sets which are similar to the unknown true result with a specified probability, we can return whole result sets, that are guaranteed to be similar (at a specified level of confidence and at a returned distance threshold) to the ground-truth.

Our solution is able to fix the gap of efficiently approximating
result-based ranking semantics, while preserving high efficiency of traditional ranking queries. %Albeit 


A solution for representative clustering of uncertain data which is related to our approach, has been presented in \cite{ZueEmrSchMametal14,schubert2015framework}. This approach takes a similar route towards finding consensus clusterings among a possibly large set of possible clusterings sampled from an uncertain database. While this approach is specialized to clustering of data, and is not trivially extendable to querying uncertain data, we borrow the concept of representing a potentially large set of possible worlds by a single result, and apply it to spatial query processing. 





\subsection{Querying Sampled Worlds}\label{sec:mc}\vspace{-0.1cm}
Let $\DB$ be an uncertain database and let $\mathcal{Q}$ be a query.
Let $X=\{X_1,...,X_{|X|}\}$ be a multiset%\footnote{Due to independent sampling, the same sample may be drawn multiple times.}
of possible worlds of
$\DB$ generated from $\DB$ using generation rule $\mathcal{G}$ and let
$\mathcal{Q}(X)$ denote the multiset of query results obtained by applying query $\mathcal{Q}$ to each
sample world in $X$. We denote the set of distinct query results in
$\mathcal{Q}(X)$ as the set $PR$ of {\em possible results} obtained from
sample $X$.
% as , $$ PC:=\{(C|C\in \mathcal{C}(X),
% n=\sum_{i=1}^{|X|}X_i={I(\mathcal{C}(X_i)=C))}\}.
% $$ $PC$.
For any result $r$ in $PR$, the {\em support} $r.support$ of $r$ is
defined as $\sum_{i=1}^{|X|}{I(\mathcal{Q}(X_i)=r)}$, where $I(\cdot)$ is an
indicator function that returns $1$ if its operand is true and $0$, otherwise.
Simply speaking, the {\em support} is the number of occurrences of
the result set $r$ in the multiset $\mathcal{Q}(X)$.
% clustering algorithm $\mathcal{C}$ applied on sample $X_i$ returns clustering
% $C$, and $0$ otherwise.
% \end{definition}
\vspace{-0.2cm}
\begin{lemma}[Approximation of the True  Result]\label{lem:approx}~\\
Under the assumptions of Definition \ref{def:uncertaindb}, for any possible
query result $r\in PR$, the probability $\hat{P}(r)=\frac{r.support}{|X|}$ is an unbiased estimator of the probability
$P(r)$ that $r$ is the true query result $\mathcal{Q}(\oracle(\DB))$ of $\DB$,
i.e., $E(\hat{P}(r))=P(r)$.
\end{lemma}
\vspace{-0.2cm}
\begin{proof}
Since the expectation of a non-random variable is the identity, we obtain
\vspace{-0.1cm}
$$
E(\hat{P}(r))=E\left(\frac{\sum_{i=1}^{|X|}I(\mathcal{Q}(X_i)=r)}{|X|}\right)=\frac{E\left(\sum_{i=1}^{|X|}I(\mathcal{Q}(X_i)=r)\right)}{|X|},
$$
Since all sample databases $X_i$ are drawn independently, and since the
expectation of a sum of independent random variables is the sum of their expectations, we get:
$$
E(\hat{P}(r))=\frac{\sum_{i=1}^{|X|} E(I(\mathcal{Q}(X_i)=r))}{|X|}
$$
Due to the assumption that each sample $X_i$ is drawn unbiased from the
distribution of all worlds of $\DB$, which implies that $E(I(\mathcal{Q}(X_i)=r))=P(r)$, we obtain \vspace{-0.2cm}
$$
\frac{\sum_{i=1}^{|X|} P(r)}{|X|}=P(r)
$$
\end{proof}


 Such a straightforward sampling approach works well for small databases. In a large
 database setting, the probability of finding exactly the same result
 on two samples in $X$ approaches zero and the probabilities $P(r)$ of a result $r$
 being the true result of $\DB$, become very small. 
 %Due to independent samplings $X_i,1\leq i\leq |X|$, the number of samples where $\mathcal{Q}(X_i)=r$ follows a binomial $B(\pi=P(r),n=|X|)$ distribution.  Estimating the probability parameter $\pi$ of a binomial distribution given a sample, requires a very large sample size $n$ if $\pi$ is small. A rule of  thumb is that $n\cdot\pi\geq 5$ \cite{CloPea34,Wal13}. 
 An exponentially large number of possible results, each associated with a marginally small probability is meaningless for a user. %A huge set of possible results, potentially exponentially large in the number of uncertain objects, and having potentially exponentially small probabilities each, where many results may be very similar is of little use.
Our approach, described in the following, clusters similar possible results in the result set space to return representative results which are similar to a large number of possible results.



\section{Representative Query Results}\label{sec:rep}\vspace{-0.0cm}
Our goal is thus to
reduce the set of possible results produced by the
Monte-Carlo approach to a small set of possible results, which are diverse and at the same time guaranteed to be similar to the result of the real (but
unknown) database. For this purpose, this section introduces a general concept
for determining representative results. First we will define a distance
function in order to measure the dissimilarity between sampled results.

\begin{definition}[result distance function (rdf)]~\\
Let $PR=\{r_1,...,r_{|PR|}\}$ denote the set of possible results derived from
sampled worlds $X=\{X_1,...,X_n\}$. Let $\rdf$ be a {\em result distance
function} $|PR|\times |PR| \rightarrow [0,1]$  such that the result of
$\rdf(r_i,r_j)$ indicates the dissimilariy between the results $r_i$ and $r_j$.
\end{definition}
An example of a simple result distance function is Jaccard distance, which measures the similarity of two results sets as used in our experimental evaluation and defined in Section~\ref{sec:evaluationmetrics}. For queries that return ranked results, a result distance function such as Kendall's rank correlation coefficient \cite{kendall1938new} or Discounted Cumulative Gain \cite{jarvelin2002cumulated} can be used to ``weigh'' ranking positions differently. 
Next, we define a representative query result as
follows:

 \begin{definition}[Representative Result]\label{def:representative}~\\
 Let $\DB$ be an uncertain database and let $\mathcal{Q}$ be a query.
 We call a query result $\mathcal{Q}(X_i)$ a $\tau\mbox{-}\phi$-representative
 result, if the probability $$
 P(X_i,\tau):=P(\rdf(\mathcal{Q}(X_i),\mathcal{Q}(\oracle(\DB)))\leq\tau) $$
  that the true (but unknown) result $\mathcal{Q}(\oracle(\DB))$ of $\DB$ has a
  distance $\rdf (\mathcal{Q}(X_i),\mathcal{C}(\oracle(\DB)))$ of at most
  $\tau$ is at least $\phi$.
 \end{definition}

Fortunately, we are able to approximate the probability $P(X_i,\tau)$ that the
true result has at most a disatance ($\rdf$) of $\tau$ by using sample results
from $\DB$:


 \begin{lemma}[Approximation of Representatives]~\\
 Let $X=\{X_1,...,X_{|X|}\}$ be a set of possible worlds of $\DB$ generated from
 $\DB$ using generation rule $\mathcal{G}$ and let $\rdf$ be a distance measure
 on result sets. Let $PR$ be the set of possible query results obtained from $X$.
The probability
$$\hat{P}(X_i,\tau):=
\frac{\sum_{j=1}^{|X|}I(\rdf(\mathcal{Q}(X_i),\mathcal{Q}(X_j))\le\tau)}{|X|}$$
 is an unbiased estimator of the probability
 $$
 P(X_i,\tau):=P(\rdf(\mathcal{Q}(X_i),\mathcal{Q}(\oracle(\DB)))\leq \tau)
 $$
 that the representative result $X_i$ has a distance of at most $\tau$ to the true query result $Q(\oracle(\DB))$.
\end{lemma}
\begin{proof}
Analogous to Lemma~\ref{lem:approx}, by substituting $\mathcal{Q}(X_i) = r$ through the
predicate $\rdf(\mathcal{Q}(X_i),r)\leq \tau$.
%$$
%E(P(C))=E(\frac{\sum_{C_i\in C}C_i.supp}{|X|})=E(\frac{\sum_{X_i\in X}\cdot I(\mathcal{D}(X_i,C)<\tau)}{|X|})
%$$
%Since the expectation of a non-random variable is the identity, we obtain
%$$
%\frac{E(\sum_{X_i\in X}\cdot I(\mathcal{D}(X_i,C)<\tau))}{|X|})
%$$
%Due to the assumption of all sample databases $X_i$ being drawn independent, and since the expectation of a sum of independent random variables is the sum of their expectations, we get
%$$
%\frac{\sum_{X_i\in X}E(I(\mathcal{D}(X_i,C)<\tau))}{|X|})
%$$
%Due to the assumption that each sample $X_i$ is drawn unbiased from the distribution of all worlds of $\DB$
%$$
%P(\mathcal{D}(C,Groundtruth(\DB))<\tau)=\sum_{w\in\mathcal{W}}I(\mathcal{D}(C,\mathcal{C}(w))<\tau)\cdot P(w)=
%$$
\end{proof}
Albeit unbiased, the probability $\hat{P}(X_i,\tau)$ cannot be used directly to assess
the probability $P(X_i,\tau)$ of result set $X_i$ having a distance of at most
$\tau$ to the true result $\mathcal{Q}(\oracle(\DB))$. Thus, $X_i$ can not
simply be returned as a $\tau\mbox{-}\phi=\hat{P}(X_i,\tau)$-representative
according to Definition~\ref{def:representative}, because the estimator
$\hat{P}(X_i,\tau)$ may overestimate the true probability $P(X_i,\tau)$. To return
$\tau$-$\phi$ representative results to the user, our aim is to find
a lower bound $\hat{P}(X_i,\tau,\alpha)$ such that we can guarantee
that $P(X_i,\tau)\geq \hat{P}(X_i,\tau,\alpha)$ with a probability of
$\alpha$, where $\alpha$ is a domain specific level of significance
(typically, $\alpha=0.95$).
% usually $\alpha\in \{0.90,0.95,0.99\}$.

To derive such a significant lower bound of $P(X_i,\tau)$ we may exploit the
fact that sampled possible worlds were drawn independently. Therefore, the
absolute number $\hat{P}\cdot |X|$ of sampled worlds which are represented by
$X_i$ follows a binomial $B(P(X_i,\tau),|X|)$ distribution. To estimate the true
probability $P(X_i,\tau)$, given realization $\hat{P}\cdot |X|$, we borrow
techniques from statistics to obtain a one sided $1-\alpha$ confidence interval
of the true probability $P(X_i,\tau)$. A simple way of obtaining such confidence
interval is by applying the central limit theorem to approximate a
binomial distribution by a normal distribution.

\begin{definition}[$\alpha$-Confidence Probabilities]\label{def:alpha}~\\
Let $\DB$ be an uncertain database. For a set of drawn database instances $X$,
and for a possible result $\mathcal{Q}(X_i),X_i\in X$, a distance threshold
$\tau$ and a level of significance $\alpha$, the probability
\begin{equation*}%\label{eq:clt}
\hat{P}(X_i,\tau,\alpha)=\hat{P}(X_i,\tau)-z\cdot\sqrt{\frac{1}{|X|}\hat{P}(X_i,\tau)\left(1-\hat{P}(X_i,\tau)\right)},
\end{equation*}
is called $\alpha$-confidence probability of $\tau$-representative $X_i$, where $z$ is the $100\cdot (1-\alpha)$ percentile of the standard normal distribution.
\end{definition}
The $\alpha$-confidence probability $\hat{P}(X_i,\tau,\alpha)$ can be used to
return the result $\mathcal{Q}(X_i)$ as a $\tau\mbox{-}\phi$-representative
query result to the user, as it guarantees, that by a user specified level of
confidence $\alpha$, the true probability $P(X_i,\tau)$ is guaranteed to be
larger than $\hat{P}(X_i,\tau,\alpha)$. To compute $\hat{P}(X_i,\tau,\alpha)$ as
in Definition~\ref{def:alpha} we argue that in our setting the central limit
theorem is applicable, since the sample size $|X|$ should be sufficiently
large ($|X|\cdot\pi\geq 5$).
Furthermore, the probability $P(X_i,\tau)$ should not be extremely small, since
a result representative having an extremely small value of $P(X_i,\tau)$ is
meaningless and should not be returned to the user in the first place. In the
case where all result representatives have an extremely small $P(X_i,\tau)$
value, the parameter $\tau$ should be increased to obtain meaningful
representatives. Yet, we note that more accurate approximations can be obtained
using Wilson Score Intervals \cite{Wil27} or using exact binomial confidence
intervals \cite{CloPea34}.


\section{Selection of Representative Results}
\label{sec:rep:select}
Using the techniques of Section \ref{sec:rep} we can estimate, for a given
$\tau$, the probability of any drawn possible world to be a
$\tau$-representative. In this section, we show how good representatives, i.e.,
possible results with a high confidence of having a low distance to a large
fraction of possible worlds, can be extracted automatically from a set of
sampled worlds. Furthermore, when more than a single representative world is
returned, a requirement is to minimize redundancy between sets of worlds
represented by each representative \cite{CuiFerDy07,JaiMekDhi08}.
This requirement is important in order to avoid overly similar result
representatives.
To solve this challenge, we propose two approaches.
The first approach requires the user to specify a maximum $\tau_{max}$ value, to
denote the maximum distance the result may have to the ground-truth to be
considered good enough. For instance, for a $10$-NN query, a user may wish to
guarantee having at least eight out of ten objects ground-truth objects
returned. Given this $\tau_{max}$ parameter, we can formulate the problem of
finding the best $\tau_{max}-\phi$-representatives as a maximum coverage problem
on the sampled results. For this $NP$-hard problem, we employ a
Greedy-approximation \cite{hochbaum1996approximating}.

Our second, parameter free approach first derives a
clustering of the set of sampled possible results $PR$ that have been obtained by applying the
any domain specific query algorithm $\mathcal{Q}$ to sampled possible worlds
$X$. Then, a single representative result $\mathcal{R}$ is chosen from each
cluster of $PR$ such that $\tau$ is minimized while the fraction of covered
drawn possible results is maximized.



\begin{algorithm}
 \caption{Maximum Cover Representatives}
   \begin{algorithmic}[1]\label{alg:cover}
       \REQUIRE {\small Level of Significance} $\alpha$, {\small Sampled Possible Results} $PR$
       \REQUIRE Similarity Threshold $\tau$, Nr. of Representatives $n$
       \STATE result = emptyset
       \FOR {$i\in 1:n$}\label{alg:cover_start}
           \STATE $\mbox{best}_r=null$
           \STATE $\mbox{best}_{\mbox{count}}=0$
           \FOR {$r \in PR$}\label{alg:cover_best1}
              \STATE covercount $= 0$
              \FOR {$r^\prime\in PR$}
                 \IF {$dist(r,r^\prime)<\tau$ }
                    \STATE covercount = covercount+1
                 \ENDIF
             \ENDFOR
             \IF {covercount $>$ $\mbox{best}_{\mbox{count}}$}
                \STATE $\mbox{best}_r=r$
             \ENDIF
           \ENDFOR\label{alg:cover_best2}
           \STATE result = result $\cap$ $(\mbox{best}_r,\tau,\hat{P}(X_i,\tau,\alpha))$\label{alg:cover_best_result}
       \ENDFOR \label{alg:cover_end}
       \RETURN result
   \end{algorithmic}
\end{algorithm}


\subsection{Maximum Representative Cover}
\label{subsec:max}
Our first approach allows a user to specify the number $n$ of representatives as
well as the maximum distance $\tau$ of a representative to the (unknown) ground
truth. Thus, this approach selects representative results such that the fraction
of possible worlds having a $\tau$-similar representative is maximized.
\begin{definition}[Maximum Cover Representatives]\label{def:max_cov}
Let $PR$ denote the set of possible query results derived from sampled worlds
$X=\{X_1,...,X_n\}$, let $\tau$ be a distance threshold, and the let $n$ be a
positive integer.
The set of maximum cover representatives $\mathcal{R}_{max}(\tau,n)\subseteq
PR$ is the set of size $n$ that maximizes the number of possible results $r\in
PR$ having a least one representative $R\in \mathcal{R}_{max}(\tau,n)$ having a
distance of at most $\tau$ to $r$. Formally:

$$
\mathcal{R}_{max}(\tau,n)=\argmax_{\mathcal{R}\subseteq PR,|R|\leq n}\sum_{r\in
PR} I(\rdf(r,\mathcal{R})\leq \tau), $$
where $I(\varphi)$ is an indicator function that returns $1$ if predicate
$\varphi$ is true and $0$ otherwise, and $\rdf(r,\mathcal{R})$ is the
minimum result distance between result $r$ and any result in $\mathcal{R}$.
\end{definition}
To find maximum cover representatives as defined in Definition
\ref{def:max_cov} an exact solution is not viable, due to the following theoretic result.
\begin{lemma}\label{lem:npcover}
The problem of computing $\mathcal{R}_{max}(\tau,n)$ is np-hard.
\end{lemma}
\begin{proof}
By reduction from the set covering problem, which is one of Karp's 21 NP-complete problems
\cite{karp1972reducibility}. Given a set of elements $U$ and a set $S$ of $n$ sets whose
union equals $U$, the set cover problem is to identify the smallest subset of S whose union
equals the universe.
For reduction to the problem of finding maximum cover representatives, map the set
$U=\{u_1,u_2,...,u_m\}$ to $PR=\{r_1,...,r_2,...,r_m\}$, map each set $s\in S$ to a
representative $r\in PR$ such that any other possible result $r^\prime\in PR$ has a distance
$dist(r,r_i)\leq \tau$ if and only if for corresponding element $u_i\in U$ it holds that
$u_i\in s$. Now, set the parameter $n$ of the maximum cover representative problem to the
smallest number of representatives able to cover all results in $PR$.
If the maximum cover representatives problem can be solved in polynomial time, then any set
covering problem can be solved in polynomial time, following the reduction above. This leads
to a contradiction assuming $P!=NP$. Thus, unless $P=NP$, the maximum cover representative
problem in np-hard.
\end{proof}

To obtain an approximate result, we employ a simple Greedy approach, which
iteratively selects the representative which covers the largest fraction of
$PR$. Following the theoretic results of \cite{hochbaum1996approximating}, this
approximation guarantees to cover $1-\frac{1}{e}\approx 0.632$ of the optimal
cover.
The algorithm of this Greedy approach is shown in Algorithm~\ref{alg:cover}.
This algorithm fetches one representative in each iteration of the loop
starting in Line \ref{alg:cover_start}. In each iteration, Lines
\ref{alg:cover_best1} - \ref{alg:cover_best2} find the possible result having the
largest fraction of $\tau$-similar results in $PR$. This result is returned as
a $\tau -\phi -$representative in Line \ref{alg:cover_best_result}, where
$\phi$ is set to an $\alpha$-significant support value according to Definition
\ref{def:alpha}.

\begin{algorithm}\label{alg:clustering}
 \caption{Possible Result Clustering}
   \begin{algorithmic}[1]
       \REQUIRE {\small Level of Significance} $\alpha$, {\small Sampled Possible Results} $PR$
       \REQUIRE Metric Clustering Algorithm $\mathcal{C}$
       \STATE result = emptyset
       \FOR {Cluster $C\in \mathcal{C}(PR)$}\label{alg:cluster_start}
           \STATE $c=\mbox{median}(C)$
           \STATE $\tau=maxDist(c,C)$
           \STATE $\phi=\hat{P}(X_i,\tau,\alpha$
           \STATE result $=result\cup (c,\tau,\phi)$
       \ENDFOR
       \RETURN result
   \end{algorithmic}
\end{algorithm}

While the maximum representative cover returns useful and intuitive result
representatives, the main drawback is the need for the user to specify the
parameters $n$ and $\tau$. The next section presents a different approach, which
allows to find a proper number of representatives, as well as the individual
similarity $\tau$ to the ground-truth adaptively for any data set.

\subsection{Possible Result Clustering}
The approach presented in Section \ref{subsec:max} requires the user to specify the data set specific parameter $\tau$. If this parameter is chosen too small, then the minimal confidence $\phi$ of the returned representatives may be extremely small. If $\tau$ is chosen too large, only a single central representative may be returned, thus loosing information about groups of mutually similar possible results.
Our second approach drops the requirement of providing any parameter. This
approach finds representative results by clustering the space of sampled results
using $\rdf$ and representing each cluster by a single representative result.
Formally:
\begin{definition}[Representative Result Clustering]
\label{def:repclust}
Let $\mathcal{C}$ be a metric clustering algorithm and let $\mathcal{C}(PR)$ denote the clustering returned by applying
$\mathcal{C}$ to the set $PR$ of possible results using $\rdf$ as distance
function. For each cluster $C \in \mathcal{C}(PR)$, a
$\tau\mbox{-}\phi$-representative result $R \in C$ is obtained. $R$ is an
$\alpha$-significant representative (cf.\ Definition~\ref{def:alpha}) with a
probability $\phi$ of at least $\hat{P}(R,\tau,\alpha)$
\end{definition}

In Definition \ref{def:repclust}, two parameters are undefined, the choice of
the clustering algorithm $\mathcal{C}$ and a heuristic to obtain a
representative from each cluster in $C\in\mathcal{C}(PR)$. For the
choice of clustering algorithm $\mathcal{C}$, we propose to use
the PAM algorithm \cite{KauRou90}, which is appropriate for general metric
spaces \cite{Jai10} but any clustering algorithm
which is appropriate for general metric spaces can be used
\cite{KauRou90,JaiMurFly99}.
% and refer to numerous clustering surveys
% \cite{JaiDub88,JaiMurFly99,KriKroZim09,Jai10,KriKroSanZim11,SimGopZimCon13}
% including metric algorithms.
For the problem of defining a representative $R$ for each a cluster $C$, we
propose to use the result that is most representative for all possible results
in a cluster $C\in \mathcal{C}(PR)$.

\begin{definition}\label{def:rep}[Cluster Representative]~\\
For a cluster $C\in \mathcal{C}(PR)$, the \emph{complete
representative} is the result $$
    R_{\text{complete}}:=\arg\min_{R\in C}\left(\max_{R^\prime\in
                                        C}\left(\rdf(R,R^\prime)\right)\right)
$$
which has the minimum maximum distance
$$
    \tau = \max_{R^\prime\in C}\left(\rdf(R,R^\prime)\right)
$$
to all other results in $C$.
\end{definition}
This representative $R$ can be returned as a
$\tau$-$\phi$-representative with confidence probability of
$\phi=\hat{P}(R,\tau,\alpha)$ using a user specified level of
confidence $\alpha$ as described in Section \ref{sec:rep}.

A drawback of the complete representative approach is that the value of
$\tau$ may grow arbitrarily large, being at least half of the corresponding
clusters diameter. A $\tau$-representative having an overly large
$\tau$ value, such as an ARI-distance \cite{HubAra85}
value greater than $0.2$, may have no semantic meaning to the user, as
the space of results represented by this $\tau$-representative grows too
large to allow meaningful decision making. Furthermore, a large value of
$\tau$ yields overlapping clusters. For instance, for a pair of complete
representatives $R_i$ and $R_j,i\neq j$, where $R_i$ is an
$\tau_i$-representative and $R_j$ is an $\tau_j$ representative, it may
hold that for a single sampled result $X_k\in X$ that
$\mathcal{D}(X_k,R_i)\leq \tau_i$ and $\mathcal{D}(X_k,R_j)\leq \tau_j$.
This drawback of complete representatives can be particularly bad, if the
underlying query algorithm $\mathcal{Q}$ is highly sensitive to changes in the database. For instance, if $\mathcal{Q}$ is a skyline algorithm, the location of single data object $o$ may dominate all of the database, rendering $o$ the only result.
In contrast, complete
representatives may yield good results in stable query settings such as $\epsilon$-range queries and $k$NN queries.

For the general case, we propose a different approach, where a maximum threshold
for $\tau$ is provided. This parameter, which is specific to the chosen distance
function $\rdf$, should be chosen in a way that a user should treat two
results, having a distance of no more than $\tau$ as
similar.
\begin{definition}[$\tau_{max}$-Clustering]~\\
Given a $\tau_{\max}$ threshold, for a cluster $C\in \mathcal{C}(PR)$ a
\emph{$\tau_{\max}$ representative} is a $\tau\mbox{-}\phi$-representative
result, such that $\tau\leq \tau_{\max}$ given by
$$
R_{\tau_{\max}}:=\arg\max_{R\in Y}\left(\sum_{C_i\in
Y}I\left(\rdf(R,C_i)\leq\tau_{\max}\right)\right)\cdot C_i.supp.
$$
\end{definition}
Again, this representative $R_{\tau_{\max}}$ can be returned as a
$\tau\mbox{-}\phi$-representative by computing a confidence probability
$\phi=\hat{P}(R_{\tau_{\max}},\tau_{\max},\alpha)$ with a user specified level
of confidence $\alpha$ as described in Definition \ref{def:rep}.

The main drawback of $\tau_{max}$ clusterings is that large fractions of
possible results may not be assigned to any $\tau$-re\-pre\-se\-nta\-tive.
The semantics of such result, however, may be useful, indicating that a large
fraction of possible results deviate too much from other results. This
indication of high heterogeneity of possible results has to be considered
when making decisions based on the uncertain data set $\DB$.

